The Resistance to Label Noise in K-NN and DNN Depends on its Concentration

We investigate the classification performance of K-nearest neighbors (K-NN) and deep neural networks (DNNs) in the presence of label noise. We first show empirically that a DNN's prediction for a given test example depends on the labels of the training examples in its local neighborhood. This motivates us to derive a realizable analytic expression that approximates the multi-class K-NN classification error in the presence of label noise, which is of independent importance. We then suggest that the expression for K-NN may serve as a first-order approximation for the DNN error. Finally, we demonstrate empirically the proximity of the developed expression to the observed performance of K-NN and DNN classifiers. Our result may explain the already observed surprising resistance of DNN to some types of label noise. It also characterizes an important factor of it showing that the more concentrated the noise the greater is the degradation in performance.

==> intro_old.tex <==
\section{Introduction} \label{sec:introduction}
% in the creation of such datasets -> when creating such
Deep neural networks (DNN) provide state-of-the-art results in many computer vision challenges, such as image classification \cite{NIPS2012_4824}, detection \cite{redmon2016yolo9000} and segmentation \cite{DBLP:journals/corr/ChenPK0Y16}. Yet, to train these models, large datasets of labeled examples are required. Time and cost limitations come into play in their creation, which often result in imperfect labeling, or \emph{label noise}, due to human error \cite{Ipeirotis10Quality}. An alternative to manual annotation are images taken from the Internet that use the surrounding text to produce labels \cite{Veit2017Learning}. This approach results in noisy labels too.

\begin{figure}
\centering
  \includegraphics[width=0.25\linewidth]{TSNE_random_cropped.png} \hspace{0.3in}
\includegraphics[width=0.25\linewidth]{TSNE_concentrated_cropped.png}
\caption{\small {\bf Effect of label noise type:} Each cluster represents a class and the color represents the label provided for each data point. (left) $20\%$ uniformly spread random noise. The network achieves $\sim100\%$ prediction accuracy. (right) $20\%$ locally concentrated noise. The network achieves $\sim80\%$ accuracy.}
\label{fig:NoiseTypes}
\end{figure}

Perhaps surprisingly, it has been shown \cite{2015arXiv151106789K} that DNNs trained on datasets with high levels of label-noise may still attain accurate predictions. This phenomenon is not unique only to DNNs but also to classic classifiers such as $K$-Nearest Neighbours ($K$-NN) \cite{Angluin88Learning, Natarajan13Learning, Frenay14Classification}.

Fig.~\ref{fig:NoiseTypes} demonstrates this behavior. It shows embeddings of deep features of the 10 MNIST classes, where we randomly change the labels of 20\% of the training data. A network trained with this data is capable of reaching $~100\%$ prediction accuracy. On the other hand, it also shows the case where concentrated groups of examples have all their labels flipped to the same label. Here too, 20\% are changed, but the noise is no longer distributed uniformly in feature space but is instead locally concentrated. In this case, the DNN does not overcome the noise and accuracy drops to $~80\%$. Clearly, the \emph{type} of label noise is as important as its \emph{amount}.

The starting point of this work is the observation that a DNN's prediction for a given test example depends on a local \emph{neighborhood} of training examples. This is motivated by recent works that show that networks perform a smooth interpolation between the labels of training examples \cite{Ongie2020Function,Savarese19How,Williams19Gradient,giryes2020function}. We suggest using  $K$-NN as a first order approximation of such an interpolation. 
We validate this assumption and empirically demonstrate that the networks' last-layer output effectively encodes the distribution of training labels in such a neighborhood, i.e., provides a similar output to a $K$-NN applied on the embedding space of the network. This may suggest that robustness bounds developed for a $K$-NN classifier applied to this space may apply also to the DNN. To this end, we develop an analytical expression that approximates the $K$-NN accuracy in the presence of randomly-spread label noise, which is of importance by itself, and show empirically that it matches the $K$-NN prediction accuracy.

Establishing the relationship between DNN and $K$-NN, we suggest that this bound may serve as a first order approximation to the accuracy of a network at different levels and types of noise. This relationship leads to an important conclusion about DNN resistance to label noise: The amount of resistance depends on how well the noisy examples are spread in the training set. When label noise is \emph{randomly spread}, the resistance is high, since the probability of noisy examples overcoming the correct ones in any local neighborhood is small. However, when the noisy examples are \emph{locally concentrated}, DNNs are unable to overcome the noise. 

We validate our analytical expression both for $K$-NN and DNN using extensive experiments on several datasets: MNIST, CIFAR-10, and ImageNet ILSVRC.
We show that empirical curves of accuracy-per-noise-level fit well with our mathematical expression. 




